TEA: Trajectory Encoding Augmentation for Robust and Transferable Policies in Offline Reinforcement Learning

In this paper, we investigate offline reinforcement learning (RL) with the goal of training a single robust policy that generalizes effectively across environments with unseen dynamics. We propose a novel approach, Trajectory Encoding Augmentation (TEA), which extends the state space by integrating latent representations of environmental dynamics obtained from sequence encoders, such as AutoEncoders. Our findings show that incorporating these encodings with TEA improves the transferability of a single policy to novel environments with new dynamics, surpassing methods that rely solely on unmodified states. These results indicate that TEA captures critical, environment-specific characteristics, enabling RL agents to generalize effectively across dynamic conditions.

==> OLD_DATA/old_files.tex <==
\subsection{Excluded (not part of paper)}
\begin{table}[H]
\centering
\caption{Average Reward on New Environment 1 (mean ± std over 10 seeds)}
\label{tab:results1std}
\begin{tabular}{lccc}
\hline
\textbf{Experiment} & \textbf{3,000 Timesteps} & \textbf{10,000 Timesteps} & \textbf{20,000 Timesteps} \\
\hline
Baseline & 121.40 ± 78.10 & 54.90 ± 49.27 & 33.00 ± 15.23 \\
AUG-ENCODING & \textbf{109.70 ± 99.36} & \textbf{93.40 ± 58.91} & \textbf{101.90 ± 73.45} \\
AUG-TRUE & 80.00 ± 64.28 & 48.70 ± 33.36 & 32.40 ± 14.42 \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N2 at 20,000 Timesteps (mean ± SEM over 10 seeds)}
\label{tab:results2}
\begin{tabular}{lc}
\hline
\textbf{Experiment} & \textbf{20,000 Timesteps} \\
\hline
Baseline & 38.50 ± 0.48 \\
AUG-ENCODING & \textbf{51.60 ± 10.31} \\
AUG-TRUE & 52.50 ± 8.72 \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N3 at 20,000 Timesteps (mean ± SEM over 10 seeds)}
\label{tab:results3}
\begin{tabular}{lc}
\hline
\textbf{Experiment} & \textbf{20,000 Timesteps} \\
\hline
Baseline & 42.50 ± 1.09 \\
AUG-ENCODING & \textbf{62.30 ± 14.82} \\
AUG-TRUE & 35.50 ± 1.38 \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N4 at 20,000 Timesteps (mean ± SEM over 10 seeds)}
\label{tab:results4}
\begin{tabular}{lc}
\hline
\textbf{Experiment} & \textbf{20,000 Timesteps} \\
\hline
Baseline & 48.50 ± 2.92 \\
AUG-ENCODING & \textbf{60.60 ± 9.63} \\
AUG-TRUE & 41.70 ± 3.89 \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N5 at 20,000 Timesteps (mean ± SEM over 10 seeds)}
\label{tab:results5}
\begin{tabular}{lc}
\hline
\textbf{Experiment} & \textbf{20,000 Timesteps} \\
\hline
Baseline & 33.10 ± 4.84 \\
AUG-ENCODING & \textbf{122.40 ± 27.95} \\
AUG-TRUE & 36.90 ± 5.99 \\
\hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{N6 at 20,000 Timesteps (mean ± SEM over 10 seeds)}
\label{tab:results6}
\begin{tabular}{lc}
\hline
\textbf{Experiment} & \textbf{20,000 Timesteps} \\
\hline
Baseline & 30.20 ± 0.49 \\
AUG-ENCODING & \textbf{43.50 ± 14.75} \\
AUG-TRUE & 30.90 ± 0.35 \\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N7 at 20.000 timesteps (mean ± SEM over 10 seeds)}
\label{tab:results7}
\begin{tabular}{lccc}
\hline
\textbf{Experiment} &\textbf{20,000 Timesteps} \\
\hline
Baseline & 45.50 ± 0.50\\
AUG-ENCODING & \textbf{55.00 ± 9.71} \\
AUG-TRUE & 43.50 ± 0.62\\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N8 at 20.000 timesteps (mean ± SEM over 10 seeds)}
\label{tab:results8}
\begin{tabular}{lccc}
\hline
\textbf{Experiment} &\textbf{20,000 Timesteps} \\
\hline
Baseline & 31.10 ± 0.64\\
AUG-ENCODING & \textbf{40.90 ± 11.38} \\
AUG-TRUE & 31.10 ± 0.57\\
\hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{N9 at 20.000 timesteps (mean ± SEM over 10 seeds)}
\label{tab:results9}
\begin{tabular}{lccc}
\hline
\textbf{Experiment} &\textbf{20,000 Timesteps} \\
\hline
Baseline & 34.80 ± 0.80\\
AUG-ENCODING & \textbf{47.10 ± 13.04} \\
AUG-TRUE & 33.80 ± 0.65\\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N10 at 20.000 timesteps (mean ± SEM over 10 seeds)}
\label{tab:results10}
\begin{tabular}{lccc}
\hline
\textbf{Experiment} &\textbf{20,000 Timesteps} \\
\hline
Baseline & 40.30 ± 0.86\\
AUG-ENCODING & \textbf{52.60 ± 13.70} \\
AUG-TRUE & 38.80 ± 0.80\\
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{N1 at 20.000 timesteps (mean ± SEM over 100 seeds)}
\label{tab:results1-100seeds}
\begin{tabular}{lccc}
\hline
\textbf{Experiment} &\textbf{20,000 Timesteps} \\
\hline
Baseline & 36.22 ± 2.16\\
AUG-ENCODING & \textbf{72.07 ± 6.64} \\
AUG-TRUE & 34.37 ± 1.56\\
\hline
\end{tabular}
\end{table}
\subsection{ToDos (not part of paper)}
\subsubsection{ToDos}
\begin{itemize}

    \item (DOING) for SEM, do /sqrt(10-1 or 100-1)



    \item (DOING) before the grid, run for 100 seeds instead of 10 seeds
    \item (Instead, refined the text description I have and added a temporary pipeline description in the end) maybe put a diagram to explain waht happens or write some pseudocode as an aglorithm or sth

    \item rotate the surface plot to show the increase better 


    \item have one big table of 10 N's where you show each result on each N1, and in last row show the average

    \item  give everyone a headsup after you are done Friday



    \item remove the blue M and the gray cloud from Figure 2.

    
\end{itemize}
\subsubsection{Final Polish}

\begin{itemize}
    \item try to fit each reference into 2 lines by using et al, shortening conference names etc
    \item maybe call it robust reinforcement learning? 
    \item make sure the tables are positioned correctly inside the paper.
    \item dont put text on top of figures, instead have it in hte captions. have the captions longer as well...
    \item choose title
    \item maybe remove contributions as a numbered list due to space constraint
\end{itemize}




\subsubsection{Done:}
\begin{itemize}
    \item Sample different points s.t.  old n8 n9 n10 which formed a line dont appear that way anymore
    \item (Instead, did interpolation with 10 points we had) have a grid with 50 points, then plot a 3d plot of the surface to show 
    \item Put carts of different sizes to our cartpole illustration
    \item Shortened related work section a bit, added  reference to LION paper.
    \item made references font size smaller (footnote) because I realized it was already small on e.g. https://arxiv.org/pdf/1907.04902
    
\end{itemize}
\subsubsection{Pipeline Description}

\paragraph{First data collection run}
\begin{enumerate}
    \item  Work on a single seed: 42

    
    \item Sample 5 source environments from 
    \begin{equation}
    \text{env\_properties} = 
    \left\{ 
    \begin{aligned}
        &\text{pole length}: \quad l_i \sim U(0.1, 2.0), \\
        &\text{cart mass}: \quad m_i \sim U(0.5, 2.0)
    \end{aligned}
    \right\}.
\end{equation}

\item Sample a new environment from the same range

\item Save respective environment properties for future reference

\item Initilize AE ( Expected input size for AE: 79 = 16*4 + 15)

\item \textbf{Prepare baseline environment: } Create a multi-environment wrapper with the 5 source environments. Each time this multi-environment wrapper resets, it will change randomly to one of the 5 environments inside it.

% \item \textbf{Prepare AUG-TRUE} Create another multi-environment wrapper with same 5 environments, yet this time, extend observation spaces with the true pole length and cart mass.

\item Train a DQN on regular cartpole environment with discrete action space (CartPole-v1)

% \item Generate replay buffer from the same regular cartpole environment using the trained DQN (this one isnt being used for anything)

\item Using the dqn trained, generate buffer for the non-augmented (baseline) multienvwrapper with source environments. Make sure to also add the id of the current env used by the multi-environment wrapper to the replay buffer for each record, s.t. you can later access them accordingly if needed.


\item Load the replay buffer you've populated on the previous step, and from that, for each source environment in the wrapper, collect trajectories of length 16. We'll use these for the sequence encoder. 

\item With the collected data, train the Autoencoder. It is being trained to recreate trajectories from a latent space dim of 4.


\item Encode each source environment with the trained autoencoder. Don't collect new data for this, but rather use the same data you've collected from step 10. Use avg. encoding of 5 trajectories to extend the observation space of each observation recorded in the replay buffer we had after step 9. Save the new replay buffer. Also save another replay buffer where you've augmented the observation space of recorded observations with the true environment parameters instead (pole length and cart mass)

\end{enumerate}

\paragraph{run bcq}

\begin{enumerate}
    \item This is done with 100 different seeds. We will use the same seed for training BCQ and evaluating on new env.
    \item Load the source and new environment properties from the data collection run (later, of course, we also tried with other 'new environment properties'). Also load the trained AE.
    \item Load the AE
    \item Encode the new environment with the AE (of course, we need to interact w/ the new environment for this.) We take 5 trajectories of length 16 and take the average encoding.

    \item BASELINE, AUG-ENCODING, AUG-TRUE: Train BCQ using data from buffers we've saved in the past using the 5 source environments. First buffer was without augmenting observation spaces, second one had augmentation with encodings, third one had augmentation with pole length and cart mass. Always train for 20.000 timesteps.

    \item Evaluate the performance on the new environment without doing any training on the new environment.

    
    
\end{enumerate}



% \begin{table}[H]
% \centering
% \caption{Average Reward on New Environment 1 (mean ± SEM over 10 seeds)}
% \label{tab:results1}
% \begin{tabular}{lccc}
% \hline
% \textbf{Experiment} & \textbf{3,000 Timesteps} & \textbf{10,000 Timesteps} & \textbf{20,000 Timesteps} \\
% \hline
% Baseline & 121.40 ± 24.70 & 54.90 ± 15.58 & 33.00 ± 4.82 \\
% AUG-ENCODING & \textbf{109.70 ± 31.42} & \textbf{93.40 ± 18.63} & \textbf{101.90 ± 23.23} \\
% AUG-TRUE & 80.00 ± 20.33 & 48.70 ± 10.55 & 32.40 ± 4.56 \\
% \hline
% \end{tabular}
% \end{table}



